Measurement of B meson production cross-sections in proton-proton collisions at sqrt(s)= 7 TeV

The production cross-sections of B mesons are measured in pp collisions at a centre-of-mass energy of 7 TeV, using data collected with the LHCb detector corresponding to a integrated luminosity of 0.36 fb-1. The B+, B0 and Bs0 mesons are reconstructed in the exclusive decays B+ -> J/psi K+, B0 -> J/psi K*0 and Bs0 -> J/psi phi, with J/psi -> mu+ mu-, K*0 -> K+ pi- and phi -> K+ K-. The differential cross-sections are measured as functions of B meson transverse momentum pT and rapidity y, in the range 0 < pT < 40 GeV/c and 2.0 < y < 4.5. The integrated cross-sections in the same pT and y ranges, including charge-conjugate states, are measured to be sigma(pp -> B+ + X) = 38.9 +- 0.3 (stat.) +- 2.5 (syst.) +- 1.3 (norm.) mub, sigma(pp -> B0 + X) = 38.1 +- 0.6 (stat.) +- 3.7 (syst.) +- 4.7 (norm.) mub, sigma(pp -> Bs0 + X) = 10.5 +- 0.2 (stat.) +- 0.8 (syst.) +- 1.0 (norm.) mub, where the third uncertainty arises from the pre-existing branching fraction measurements.

==> preamblebak.tex <==
% THis file contains all the default packages and modifications for
% LHCb formatting

%% %%%%%%%%%%%%%%%%%%
%%  Page formatting
%% %%%%%%%%%%%%%%%%%%
\textheight=230mm
\textwidth=160mm
\oddsidemargin=7mm
\evensidemargin=-10mm
\topmargin=-10mm
\headsep=20mm
\columnsep=5mm
\addtolength{\belowcaptionskip}{0.5em}

\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.99}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}


\setlength{\hoffset}{-2cm}
\setlength{\voffset}{-2cm}
% Page defaults ...
\topmargin=0.5cm
\oddsidemargin=2.5cm
\textwidth=16cm
\textheight=22cm
% Allow the page size to vary a bit ...
\raggedbottom
% To avoid Latex to be too fussy with line breaking ...
\sloppy

%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%%
\usepackage{microtype}
\usepackage{lineno}  % for line numbering during review
\usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbol
%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
\usepackage{color}
\usepackage{colortbl}
\graphicspath{{./figs/}} % Make Latex search fig subdir for figures
%\usepackage{rotating}

%% Math
\usepackage{amsmath} % Adds a large collection of math symbols
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

\usepackage{booktabs}
\usepackage{multirow}
%\usepackage{times}
\usepackage{multirow}
\usepackage{mathptmx}
\usepackage{rotating}
%\usepackage[T1]{fontenc}
%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/viewtopic.php?f=5&t=163
%%
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
\expandafter\let\csname oldend#1\expandafter\endcsname\csname
end#1\endcsname
 \renewenvironment{#1}%
   {\linenomath\csname old#1\endcsname}%
   {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.
\usepackage{hyperref}    % Hyperlinks in references
\usepackage[all]{hypcap} % Internal hyperlinks to floats.
\usepackage{booktabs,threeparttable}
%\usepackage{amssymb}
%\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset
%\usepackage{mciteplus}
% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.
\usepackage{hyperref}    % Hyperlinks in references
\usepackage[all]{hypcap} % Internal hyperlinks to floats.
\usepackage[below]{placeins} % clean float before section
%\usepackage[below]{placeins}
\DeclareMathAlphabet{\mathbfi}{OT1}{ptm}{bx}{it}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\input{lhcb-symbols-def} % Add in the predefined LHCb symbols

% Make this the last packages you include before the \begin{document}
\usepackage{cite} % Allows for ranges in citations
\usepackage{mciteplus}

\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}

\newcommand{\pbinv}{\invpb}
\newcommand{\ptrans}{\ensuremath{p_{\rm T}}}
\newcommand{\bpjpsipi}{\ensuremath{\bplus\to\jpsi \pi^+}}
\newcommand{\jpsimumu}{\ensuremath{\jpsi\to\mu^+ \mu^-}}
\newcommand{\bsubc}{\ensuremath{B_c^+}}
\newcommand{\bplus}{\ensuremath{B^{\rm +}}}
\newcommand{\bzero}{\ensuremath{B^{\rm 0}}}
\newcommand{\bszero}{\ensuremath{B^{\rm 0}_s}}
\newcommand{\bcjpsipi}{\ensuremath{\bsubc\to\jpsi\pi^+}}
\newcommand{\bpjpsik}{\ensuremath{\bplus\to\jpsi K^+}}
\newcommand{\bzjpsikstar}{\ensuremath{\bzero\to\jpsi K^{*0}}}
\newcommand{\kstar}{\ensuremath{K^{*0}}}
\newcommand{\kstarkpi}{\ensuremath{\kstar\to K^+\pi^-}}
\newcommand{\bzjpsiks}{\ensuremath{\bzero\to\jpsi K^0_s}}
\newcommand{\bszjpsiphi}{\ensuremath{\bszero\to\jpsi \phi}}
\newcommand{\phikk}{\ensuremath{\phi\to K^+K^-}}
\newcommand{\cndof}{\ensuremath{\chi^2/{\rm ndf}}}
\newcommand{\bpyyresult}{\ensuremath{38.9\pm0.3\,({\rm stat.})\pm2.8\,({\rm syst.})\,{\rm \mub}}}
\newcommand{\bpyynobrresult}{\ensuremath{38.9\pm0.3\,({\rm stat.})\pm2.5\,({\rm syst.})\,\pm1.3({\rm norm.})\,{\rm \mub}}}
%\newcommand{\bzresult}{\ensuremath{38.9\pm0.6\,({\rm stat.})\pm3.6\,({\rm syst.})\,\pm4.8({\rm norm.})\,{\rm \mub}}}
\newcommand{\bzresult}{\ensuremath{38.1\pm0.6\,({\rm stat.})\pm3.7\,({\rm syst.})\,\pm4.7({\rm norm.})\,{\rm \mub}}}
\newcommand{\bszresult}{\ensuremath{10.5\pm0.2\,({\rm stat.})\pm0.8\,({\rm syst.})\pm1.0\,({\rm norm.})\,{\rm \mub}}}
\newcommand{\bszbrresult}{\ensuremath{11.0\pm0.3\,({\rm stat.})\pm0.8\,({\rm syst.})\,{\rm nb}}}

\newcommand{\bxs}{$B$ meson production cross-section}
\newcommand{\bxss}{\bxs s}
\newcommand{\Bxs}{$B$ meson production cross-section}
\newcommand{\allbxs}{$B$ meson production cross-section}
\newcommand{\allbxss}{\allbxs s}
\newcommand{\bmeson}{$B$ meson}
\newcommand{\reald}{real data}
\newcommand{\bmesons}{\bmeson s}
\newcommand{\sm}{\mbox{Standard} \mbox{Model}}
\newcommand{\divv}{{\rm d}}
\newcommand{\alphas}{\ensuremath{\alpha_s}}
\newcommand{\mur}{\ensuremath{\mu_{\rm R}}}
\newcommand{\muf}{\ensuremath{\mu_{\rm F}}}
\newcommand{\sweight}{\ensuremath{\it _sWeight}}
\newcommand{\sweights}{\ensuremath{\it _sWeights}}
\newcommand{\splot}{\ensuremath{\it _s Plot}}
\newcommand{\lagrangian}{{\cal L}{\rm agrangian}}
\newcommand{\lumivalue}{\ensuremath{0.36\pm0.01\invfb}}
\newcommand{\lumionly}{\ensuremath{0.36\invfb}}
\newcommand{\ppsymbol}{\ensuremath{pp}}
%\newcommand{\lumivalue}{\ensuremath{362\pm13\pbinv}}
%\newcommand{\lumionly}{\ensuremath{362\pbinv}}

